SkyGrid: Energy-Flow Optimization at Harmonized Aerial Intersections

The rapid evolution of urban air mobility (UAM) is reshaping the future of transportation by integrating aerial vehicles into urban transit systems. The design of aerial intersections plays a critical role in the phased development of UAM systems to ensure safe and efficient operations in air corridors. This work adapts the concept of rhythmic control of connected and automated vehicles (CAVs) at unsignalized intersections to address complex traffic control problems. This control framework assigns UAM vehicles to different movement groups and significantly reduces the computation of routing strategies to avoid conflicts. In contrast to ground traffic, the objective is to balance three measures: minimizing energy utilization, maximizing intersection flow (throughput), and maintaining safety distances. This optimization method dynamically directs traffic with various demands, considering path assignment distributions and segment-level trajectory coefficients for straight and curved paths as control variables. To the best of our knowledge, this is the first work to consider a multi-objective optimization approach for unsignalized intersection control in the air and to propose such optimization in a rhythmic control setting with time arrival and UAM operational constraints. A sensitivity analysis with respect to inter-platoon safety and straight/left demand balance demonstrates the effectiveness of our method in handling traffic under various scenarios.

==> 2_Related_Works.tex <==
% \section{Related Works}



%  With increasing demand for aerial transportation, especially for large urban and inter-urban distances, a significant time of UAM flights would include cruising at a fixed altitude \cite{johnson2022nasa}.  Although large altitude variations are prohibited through this cruising phase, and can cause inter-vehicle conflicts in heterogeneous urban environments, vehicles can benefit from a limited altitude variation range, offering more space for routing vehicles of different movement groups at aerial intersections. Moreover, as there has been extensive study on intersection control on the ground \red{(REF)},  many ideas can be borrowed for aerial intersection control.








% \subsection{\textit{\textbf{Unsignalized Intersection Control}}}

%  Several factors makes a shared airspace a potential environment for unsignalized routing and intersection control. Many restrictions such as predefined lanes and intersection structure, limited turning zones, restrict motion control on the ground. Unsignalized intersections in the air provide the opportunity of controlling CAVs with less uncertainties which are common on the ground such as road imperfections, obstacles, etc.  Morevoer, the air offers a more flexible space with lower uncertainty from environmental variables, more control capacity, and the possibility of a hierarchical design in abstract components of intersection control such as the main intersection volume and graph as well as  detailed design of the path and trajectories vehicles should accurately follow. In other works, we can view unsignalized intersection control in an open 3D space as a larger path planning problem from the graph level design, down to the path level design. Fig. \ref{fig:intersection_design_levels} represents a hierarchical design for a general intersection control problem. 






% \subsection{\textit{\textbf{Multi-objective Optimization}}}

% \cite{kumaravel2021optimal} and \cite{jiang2022coordination} propose a similar approach to our work, for ground intersection control, \cite{jiang2022coordination} controls the entry time of a virtual platoon at a conflicting intersection on the upper level to minimize the total delay of the intersection, while minimizing the energy in a lower level optimal control problem called eco-driving strategy.  However, they rely on the L2 norm of the control variable which is the speed as the cost function, which only represents the kinetic energy at straight segments. However, in our case considering the air resistance at high speeds  (for light aerial vehicles) is necessary when calculating the required energy for a movement. In our work, the L2 norm of the control variable, which in \cite{kumaravel2021optimal}, \cite{jiang2022coordination} is used as the cost function representing energy consumption, is no longer accurate and the energy should be derived from scratch in every scenario. 

% \red{Should finish with summing up limitations of previous work and justification of current work}









